Beyond Nyquist: Efficient Sampling of Sparse Bandlimited Signals

Wideband analog signals push contemporary analog-to-digital conversion systems to their performance limits. In many applications, however, sampling at the Nyquist rate is inefficient because the signals of interest contain only a small number of significant frequencies relative to the bandlimit, although the locations of the frequencies may not be known a priori. For this type of sparse signal, other sampling strategies are possible. This paper describes a new type of data acquisition system, called a random demodulator, that is constructed from robust, readily available components. Let K denote the total number of frequencies in the signal, and let W denote its bandlimit in Hz. Simulations suggest that the random demodulator requires just O(K log(W/K)) samples per second to stably reconstruct the signal. This sampling rate is exponentially lower than the Nyquist rate of W Hz. In contrast with Nyquist sampling, one must use nonlinear methods, such as convex programming, to recover the signal from the samples taken by the random demodulator. This paper provides a detailed theoretical analysis of the system's performance that supports the empirical observations.

==> bios.tex <==
\begin{biographynophoto}{Joel A.\ Tropp}
(S'03, M'04) earned the B.A.\ degree in Plan II Liberal Arts Honors and the B.S.\ degree in Mathematics from the University of Texas at Austin in 1999, graduating \emph{magna cum laude}.  He continued his graduate studies in Computational and Applied Mathematics (CAM) at UT-Austin where he completed the M.S.\ degree in 2001 and the Ph.D.\ degree in 2004.  His graduate work was supported by an NSF Graduate Fellowship and a CAM Graduate Fellowship.

In 2004, Dr.\ Tropp joined the Mathematics Department of the University of Michigan at Ann Arbor as Research Assistant Professor.  In 2005, he won an NSF Mathematical Sciences Postdoctoral Research Fellowship, and he was appointed T.\ H.\ Hildebrandt Research Assistant Professor.  Since August 2007, Dr.\ Tropp has been Assistant Professor of Computational and Applied Mathematics at the California Institute of Technology.  He is recipient of an ONR Young Investigator Award (2008) and a Presidential Early Career Award for Scientists and Engineers (PECASE 2009).
\end{biographynophoto}


\begin{biographynophoto}{Jason N.\ Laska}
\end{biographynophoto}

\begin{biographynophoto}{Marco F.\ Duarte}
(S'99, M'09) received the B.S.\ degree in Computer Engineering (with distinction) and the M.S.\ degree in Electrical Engineering from the University of Wisconsin at Madison in 2002 and 2004, respectively, and the Ph.D.\ degree in Electrical Engineering from Rice University in 2010. He is currently an NSF/IPAM Mathematical Sciences Postdoctoral Research fellow in the Program of Applied and Computational Mathematics at Princeton University. His research interests include machine learning, compressive sensing, sensor networks, and optical image coding. He received the Presidential Fellowship and the Texas Instruments Distinguished Fellowship in 2004 and the Hershel M.\ Rich Invention Award in 2007, all from Rice University. He is also a member of Tau Beta Pi and SIAM.
\end{biographynophoto}

\begin{biographynophoto}{Justin K.\ Romberg}
is Assistant Professor in the School of Electrical
and Computer Engineering at the Georgia Institute of Technology.  Dr.\ Romberg
received the B.S.E.E.\ (1997), M.S.\ (1999) and Ph.D.\ (2003) degrees from Rice University in Houston, Texas.  From Fall 2003 until Fall 2006, he was Postdoctoral Scholar in Applied and Computational Mathematics at the California Institute of Technology.  He spent the Summer of 2000 as a researcher at Xerox PARC, the Fall of 2003 as a visitor at the Laboratoire Jacques-Louis Lions in Paris, and the Fall of 2004 as a Fellow at the UCLA Institute for Pure and Applied Mathematics (IPAM).  In the Fall of 2006, he joined the ECE faculty as a member of the Center for Signal and Image Processing.  He received an ONR Young Investigator Award in 2008, and a PECASE award in 2009.  He is also currently an Associate Editor for the {\sl IEEE Transactions on Information Theory}.
\end{biographynophoto}

\begin{biographynophoto}{Richard G.\ Baraniuk}
\end{biographynophoto}
